A Comprehensive Study of Governance Issues in Decentralized Finance Applications

Decentralized Finance (DeFi) is a prominent application of smart contracts, representing a novel financial paradigm in contrast to centralized finance. While DeFi applications are rapidly emerging on mainstream blockchain platforms, their quality varies greatly, presenting numerous challenges, particularly in terms of their governance mechanisms. In this paper, we present a comprehensive study of governance issues in DeFi applications. Drawing upon insights from industry reports and academic research articles, we develop a taxonomy to categorize these governance issues. We collect and build a dataset of 4,446 audit reports from 17 Web3 security companies, categorizing their governance issues according to our constructed taxonomy. We conducted a thorough analysis of governance issues and identified vulnerabilities in governance design and implementation, e.g., voting sybil attack and proposal front-running. Our findings highlight a significant observation: the disparity between smart contract code and DeFi whitepapers plays a central role in these governance issues. As an initial step to address the challenges of code-whitepaper consistency checks for DeFi applications, we built a machine-learning-based prototype, and validated its performance on eight widely used DeFi projects, achieving a 56.14% F1 score and a 80% recall. Our study culminates in providing several key practical implications for various DeFi stakeholders, including developers, users, researchers, and regulators, aiming to deepen the understanding of DeFi governance issues and contribute to the robust growth of DeFi systems.

==> sections/motivation.tex <==
%\todo{introduce why we do this study}
% Decentralized finance~(DeFi) is one of the major applications of the smart contract and is a novel finance paradigm in contrast to centralized finance. DeFi allows users to bypass intermediaries, such as banks, and transact directly. On mainstream blockchain platforms, decentralized finance applications~(DeFi Apps) are emerging in large numbers, but quality varies widely, facing many challenges, especially in terms of governance in the smart contract. DeFi Apps are one special type of software implemented in smart contracts. Its governance is different from conventional application lifecycle management~(ALM)~\cite{kaariainen2009applying,rossberg2014beginning}
%although initially, DeFi Apps has the same development and deployment process as traditional applications. %A core team designs, implements, tests, and releases the DeFi application. 

\cz{Why not merge this section with intro?}

% Decentralized Finance (DeFi) is one of the main applications of smart contracts and represents a novel financial paradigm in contrast to centralized finance. DeFi enables users to bypass intermediaries such as banks and participate directly in transactions. On mainstream blockchain platforms, numerous DeFi applications~(DeFi Apps) are emerging, but their quality varies, especially in terms of governance of smart contracts. DeFi Apps are a specific type of software implemented within smart contracts. \textbf{First}, Decentralized Finance (DeFi) applications, once deployed on a blockchain, exhibit immutable characteristics; their code cannot be modified post-deployment. This makes the maintenance of DeFi applications, which includes tasks such as bug fixes or feature enhancements, more challenging than for traditional softwares. \textbf{Second}, smart contracts are designed to programmatically implement the contractual clauses delineated by the development team in the whitepaper. To remain true to the promises made to the users, smart contracts must adhere to these clauses permanently. Any discrepancy between the promises of the white paper and the implementation of smart contracts can be perceived as a breach of contract. Any modifications to the contractual clauses should be ratified by the user community, thereby ensuring the protection of users' rights and interests. Unilateral changes that do not honor the consensus of the community violate the principle of decentralization.

%\cz{missing: one example demonstrating a governance issue and its consequence.}

%\cz{missing: some statistics showing that governance is something DApp developers care about, or showing that governance issue is one of the major issues.}
%For example, Audius Governance Takeover~\footnote{https://blog.audius.co/article/audius-governance-takeover-post-mortem-7-23-22} is caused by one inconsistency with the contract updating mechanism so that the attacker can change the admin address. Fixing this vulnerability involves a lot of effort, and all contracts were re-deployed.

The governance of Decentralized Finance (DeFi) applications plays a critical role in DeFi activities. \revise{The failure of DeFi governance can result in substantial financial losses for its users. For example, ARBIX FINANCE claims that users can gain optimal yield with the low risk. However, the ownership of the ARBIX FINANCE~\footnote{https://cointelegraph.com/news/certik-identifies-arbix-finance-as-a-rug-pull-warns-users-to-steer-clear}{} implementation belongs to only one owner and can be minted arbitrarily. This contradicts the claimed low risk. In the end, ARBIX FINANCE absconded with a substantial sum of 10 million dollars. Another example is Beanstalk~\footnote{https://a16zcrypto.com/posts/article/dao-governance-attacks-and-how-to-avoid-them/}. The governance design flaw makes itself vulnerable to the governance attack through flashloan.}

Despite its significance, the sphere of DeFi application governance has been relatively understudied, and it is imperative to identify prominent challenges, evaluate existing solutions, and propose potential future strategies. Although there exist numerous studies on blockchain governance, they tend to primarily focus on a high-level, theoretical delineation of the term governance, neglecting the pragmatic governance issues that arise in real-world applications. This disparity creates a gap between academia and industry. Our research signifies a pioneering attempt to examine the governance of DeFi applications comprehensively, drawing on auditing reports provided by relevant entities. \revise{Our study aims to figure out what challenges the governance faces, what are the governance issues, and what solution to address them.}
